Piecewise Planar Hulls for Semi-Supervised Learning of 3D Shape and Pose from 2D Images

We study the problem of estimating 3D shape and pose of an object in terms of keypoints, from a single 2D image. The shape and pose are learned directly from images collected by categories and their partial 2D keypoint annotations.. In this work, we first propose an end-to-end training framework for intermediate 2D keypoints extraction and final 3D shape and pose estimation. The proposed framework is then trained using only the weak supervision of the intermediate 2D keypoints. Additionally, we devise a semi-supervised training framework that benefits from both labeled and unlabeled data. To leverage the unlabeled data, we introduce and exploit the \emph{piece-wise planar hull} prior of the canonical object shape. These planar hulls are defined manually once per object category, with the help of the keypoints. On the one hand, the proposed method learns to segment these planar hulls from the labeled data. On the other hand, it simultaneously enforces the consistency between predicted keypoints and the segmented hulls on the unlabeled data. The enforced consistency allows us to efficiently use the unlabeled data for the task at hand. The proposed method achieves comparable results with fully supervised state-of-the-art methods by using only half of the annotations. Our source code will be made publicly available.

==> conclusion.tex <==
% \newpage
\section{Conclusion}
We proposed a semi-supervision framework for 3D shape and pose estimation in terms of keypoints. In this framework, a model is trained with limited 2D keypoint annotations, which at test time can estimate the 3D shape and pose directly from a single image. To achieve this, we propose \emph{piecewise planar hulls} which are structures that form a bridge between semantic segmentation and keypoint estimation. This relationship allowed us to derive the self-supervision loss, thereby enabling us to efficiently use unlabelled data. The proposed self-supervision relies on the pseudo-labels derived from the predictions and the cross-consistency between them. In this work, we also presented an exploration-exploitation technique to effectively generate pseudo-targets for 2D keypoints from segmentation pseudo-labels using piecewise planar hulls. The experiments show that the proposed framework consistently offers very promising results compared to the baseline and the state-of-the-art methods. In the  semi-supervised setting, it achieves comparable results with fully supervised state-of-the-art methods by using only half of the annotations. 
 

